Causal SHAP: Feature Attribution with Dependency Awareness through Causal Discovery

Explaining machine learning (ML) predictions has become crucial as ML models are increasingly deployed in high-stakes domains such as healthcare. While SHapley Additive exPlanations (SHAP) is widely used for model interpretability, it fails to differentiate between causality and correlation, often misattributing feature importance when features are highly correlated. We propose Causal SHAP, a novel framework that integrates causal relationships into feature attribution while preserving many desirable properties of SHAP. By combining the Peter-Clark (PC) algorithm for causal discovery and the Intervention Calculus when the DAG is Absent (IDA) algorithm for causal strength quantification, our approach addresses the weakness of SHAP. Specifically, Causal SHAP reduces attribution scores for features that are merely correlated with the target, as validated through experiments on both synthetic and real-world datasets. This study contributes to the field of Explainable AI (XAI) by providing a practical framework for causal-aware model explanations. Our approach is particularly valuable in domains such as healthcare, where understanding true causal relationships is critical for informed decision-making.

==> Results_Archive.tex <==
% Main Results Table
\section{Results and Discussion}

\subsection{Synthetic Datasets}
\subsubsection{Cardiovascular Disease}
In this test dataset, there are 1000 samples and 5 features: diet score, BMI, age, fitness, and exercise level, with cardiovascular risk as the target variable. BMI depends on diet score and age, where $\mu_{\text{bmi},i} = 25 + 0.7 \cdot z(\text{age}_i) + 0.8 \cdot z(\text{diet\_score}_i)$. Fitness depends on age and exercise level, where $\mu_{\text{fitness},i} = 7 + 0.7 \cdot z(\text{age}_i) + 0.8 \cdot z(\text{exercise\_level}_i)$. Finally, the target cardiovascular risk depends on BMI, age and fitness, where $\mu_{\text{cv\_risk},i} = 0.8 \cdot z(\text{bmi}_i) + 0.8 \cdot z(\text{age}_i) + 0.8 \cdot z(\text{fitness}_i)$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{Images/Synthetic_CV.png}
    \caption{Causal Edges in Synthetic Cardiovascular Disease Dataset}
    \label{fig:enter-label}
\end{figure}

\subsubsection{Lung Cancer}
In this test dataset, there are 1000 samples and 5 features: age, smoking, air pollution exposure, air quality index, and industrial activity, with lung cancer risk as the target variable. The air quality index depends on air pollution exposure and industrial activity, where $\mu_{\text{air\_quality\_index},i} = 20 + 0.8 \cdot z(\text{air\_pollution\_exposure}_i) + 0.5 \cdot z(\text{industrial\_activity}_i)$. Lung cancer risk depends on age, smoking, and air quality index, where $\mu_{\text{lung\_cancer\_risk},i} = \mu_{\text{lung\_cancer\_risk\_mean},i} + \text{rnorm}(n\_samples, 0, \mu_{\text{lung\_cancer\_risk\_std},i})$, with $\mu_{\text{lung\_cancer\_risk\_mean},i} = 0.001 \cdot \text{age}_i^2 + 0.2 \cdot \text{smoking}_i + 0.3 \cdot \mu_{\text{air\_quality\_index},i}$ and $\mu_{\text{lung\_cancer\_risk\_std},i} = 2 + 0.1 \cdot \text{age}_i + 0.05 \cdot \text{smoking}_i + 0.05 \cdot \text{air\_pollution\_exposure}_i$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{Images/Synthetic_LC.png}
    \caption{Causal Edges in Synthetic Lung Cancer Dataset}
    \label{fig:enter-label}
\end{figure}

\subsection{Evaluation Method}
For synthetic dataset, we observe that there is a lack of standardized evaluation metrics for causality integration in XAI techniques. Hence, we propose a new custom evaluation method to quantify the effectiveness of our algorithm. In this evaluation method, we will have three steps. Firstly, we compute feature attributions on all features using two approaches: Causal SHAP and a baseline SHAP implementation (either Kernel SHAP or Tree SHAP). Next, we calculate the exact SHAP values by considering all possible feature coalitions on a subset of the features. Specifically, we exclude intermediary features that lie along causal paths. For example, $A->B->C$ where C is the target variable, we will exclude B in the second step and only compute exact SHAP score only for the effect of A on C. In our third step, we will compare the attribution values from step 1 with those from step 2 using root mean squared error (RMSE). A lower RMSE indicates better capture of causal relationships, as it shows the method's attributions better match those computed when intermediary features are removed. This alignment suggests the method effectively accounts for causal path in its original attributions. 


\subsection{Results on Synthetic Datasets}
\begin{table}[H]
\centering
\caption{Evaluation Results: RMSE Between Full and Reduced Feature Set Attributions}
\label{tab:causal_eval}
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Kernel SHAP} & \textbf{Tree SHAP} & \textbf{Causal SHAP} \\
\midrule
Synthetic 1 & 0.4172 $\pm$ 0.0242  & 0.3213 $\pm$ 0.0190 & \textbf{0.2520 $\pm$ 0.0631} \\
Synthetic 2 & 2.4736 $\pm$ 0.1554  & 2.4935 $\pm$ 0.1485 & \textbf{2.3455 $\pm$ 0.2541} \\
\bottomrule
\end{tabular}
\end{table}


\begin{table*}[t]
\centering
\caption{Main Results: Comparison of Global Feature Attribution Methods}
\label{tab:main-results}
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{Insertion Score} & \multicolumn{3}{c}{Deletion Score} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& AUROC & Cross Entropy & Brier & AUROC & Cross Entropy & Brier \\
\midrule
\multicolumn{7}{l}{\textbf{Real-world Datasets}} \\
\midrule
IBS & & & & & & \\
- Kernel SHAP & $0.85486 \pm 0.02849$ & $0.46743 \pm 0.03603$ & $0.14747 \pm 0.01484$ & $0.61556 \pm 0.02501$ & $\underline{0.80445 \pm 0.03240}$ & $\underline{0.30158 \pm 0.01505}$ \\
- Tree SHAP & $0.85501 \pm 0.02817$ & $0.46717 \pm 0.03577$ & $0.14740 \pm 0.01472$ & $0.60957 \pm 0.03264$ & $0.80368 \pm 0.02820$ & $0.30121 \pm 0.01312$ \\
- Causal SHAP & $\underline{0.85941 \pm 0.02272}$ & $\underline{0.46454 \pm 0.03148}$ & $\underline{0.14646 \pm 0.01347}$ & $\underline{0.59925 \pm 0.04507}$ & $0.80119 \pm 0.04598$ & $0.29941 \pm 0.02055$ \\
Lung Cancer & & & & & & \\
- Kernel SHAP & $0.71056 \pm 0.02151$ & $0.63781 \pm 0.02376$ & $0.22078 \pm 0.00902$ & $0.52335 \pm 0.01253$ & $0.81659 \pm 0.07136$ & $0.30112 \pm 0.02745$ \\
- Tree SHAP & $\underline{0.71103 \pm 0.02158}$ & $\underline{0.63712 \pm 0.02411}$ & $\underline{0.22058 \pm 0.00910}$ & $\underline{0.52278 \pm 0.01290}$ & $\underline{0.81726 \pm 0.07040}$ & $\underline{0.30142 \pm 0.02707}$ \\
- Causal SHAP & $0.70579 \pm 0.01730$ & $0.64224 \pm 0.02234$ & $0.22270 \pm 0.00814$ & $0.53621 \pm 0.01408$ & $0.79184 \pm 0.06003$ & $0.29130 \pm 0.02400$ \\
[0.5em]
Colorectal Cancer & & & & & & \\
- Kernel SHAP & $0.62633 \pm 0.01492$ & $0.67666 \pm 0.00909$ & $0.24101 \pm 0.00404$ & $0.54079 \pm 0.02233$ & $0.69485 \pm 0.00614$ & $0.25069 \pm 0.00297$ \\
- Tree SHAP & $0.62651 \pm 0.01560$ & $0.67655 \pm 0.00948$ & $0.24097 \pm 0.00418$ & $\underline{0.53948 \pm 0.02139}$ & $\underline{0.69510 \pm 0.00618}$ & $\underline{0.25082 \pm 0.00301}$ \\
- Causal SHAP & $\underline{0.62716 \pm 0.01904}$ & $\underline{0.67355 \pm 0.00969}$ & $\underline{0.23972 \pm 0.00440}$ & $0.55344 \pm 0.00933$ & $0.69102 \pm 0.00446$ & $0.24882 \pm 0.00214$ \\   

\toprule
& \multicolumn{3}{c}{Insertion Score} & \multicolumn{3}{c}{Deletion Score} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& RMSE & MAE & R^2 & RMSE & MAE & R^2 \\
\midrule
\multicolumn{7}{l}{\textbf{Synthetic Datasets}} \\
\midrule
Cardiovascular & & & & & & \\
- Kernel SHAP & $1.01493 \pm 0.03098$ & $0.87613 \pm 0.02927$ & $0.49700 \pm 0.043952$ & $4.20022 \pm 0.089142$ & $3.80881 \pm 0.07828$ & $-3.91218 \pm 0.30400$\\
- Tree SHAP & $1.01509 \pm 0.03102$ & $0.87625 \pm 0.02930$ & $0.49697 \pm 0.04400$ & $\underline{4.20145 \pm 0.08819}$ & $\underline{3.80997 \pm 0.07776}$ & $\underline{-3.91567 \pm 0.30865}$ \\
- Causal SHAP & $\underline{1.01261 \pm 0.03573}$ & $\underline{0.87481 \pm 0.03352}$ & $\underline{0.49881 \pm 0.04651}$ & $4.18568 \pm 0.05800$ & $3.79633 \pm 0.05947$ & $-3.88944 \pm 0.35343$ \\
[0.5em]
Lung Cancer & & & & & & \\
- Kernel SHAP & \underline{$10.2857 \pm 0.58775$} & $\underline{8.05049 \pm 0.40233}$ & $\underline{0.33604 \pm 0.03598}$ & $\underline{24.3909 \pm 1.11470}$ & $\underline{21.2610 \pm 1.17275}$ & $\underline{-2.78584 \pm 0.59145}$ \\
- Tree SHAP & $\underline{10.2857 \pm 0.58775}$ & $\underline{8.05049 \pm 0.40233}$ & $\underline{0.33604 \pm 0.03598}$ & $\underline{24.3909 \pm 1.11470}$ & $\underline{21.2610 \pm 1.17275}$ & $\underline{-2.78584 \pm 0.59145}$ \\
- Causal SHAP & $10.3378 \pm 0.54926$ & $8.06827 \pm 0.32372$ & $0.32874 \pm 0.03306$ & $23.4773 \pm 0.84150$ & $20.3593 \pm 0.88991$ & $-2.50664 \pm 0.48840$ \\
\bottomrule
\end{tabular}
\small
\begin{tablenotes}
\item[1] All results are averaged over 5 runs with different random seeds. $\mu$ represents the mean and $\sigma$ represents the standard deviation.
\item[2] Underline values indicate the best performance for each dataset and metric.
\end{tablenotes}
\end{table*}

==> references.tex <==
\bibliographystyle{IEEEtran}
\bibliography{references}


